Modeling Associative Reasoning Processes

The human capability to reason about one domain by using knowledge of other domains has been researched for more than 50 years, but models that are formally sound and predict cognitive process are sparse. We propose a formally sound method that models associative reasoning by adapting logical reasoning mechanisms. In particular it is shown that the combination with large commensense knowledge within a single reasoning system demands for an efficient and powerful association technique. This approach is also used for modelling mind-wandering and the Remote Associates Test (RAT) for testing creativity. In a general discussion we show implications of the model for a broad variety of cognitive phenomena including consciousness.

==> planung <==
Im Moment starten wir ja gleich mit Bewusstsein. Die eigentliche Anwendung mit Assoziationen kommt erst viel später. Ich habe verstanden, dass wir das umdrehen wollen. Ich schlage vor:

\textbf{Einleitung} 

\begin{itemize}
\item bisher gibt es keine Ansätze zur Modellieren von assoziativem Denken 
\item diese waeren auch im KI Bereich auch interessant 
\item Wir starten mit Commonsense Reasoning Beispiel.
\item Dazu braucht man Wissen - was gibt es da ...
\item Dazu brauchen wir auch assoziatives Denken (durch COPA Beispiel motivieren)
\item Traditionelle Reasoning Techniken scheitern da ---- SINE usw
\item Wir schlagen Assoziationstechniken vor, wie sie wohl auch Menschen benutzen: Und schon sind wir bei word embeddings. Das das nützlich ist, haben wir schon im CADE Paper "Names" gezeigt.
\end{itemize}
}
\textbf{Alter Abschnitt 3 Automated Reasoning and Global Workspace Theory}

aber ohne Bezug zur GWT

\textbf{Alter Abschnitt 2 Information and Consciousness}
dabei alten Abschnitt 4 einarbeiten. Der Abschnitt könnte aber auch nach hinten, nach Creativity

\textbf{Mind Wandering}

\textbf{Creativity}

